Robust Iris Segmentation Based on Fully Convolutional Networks and Generative Adversarial Networks

The iris can be considered as one of the most important biometric traits due to its high degree of uniqueness. Iris-based biometrics applications depend mainly on the iris segmentation whose suitability is not robust for different environments such as near-infrared (NIR) and visible (VIS) ones. In this paper, two approaches for robust iris segmentation based on Fully Convolutional Networks (FCNs) and Generative Adversarial Networks (GANs) are described. Similar to a common convolutional network, but without the fully connected layers (i.e., the classification layers), an FCN employs at its end a combination of pooling layers from different convolutional layers. Based on the game theory, a GAN is designed as two networks competing with each other to generate the best segmentation. The proposed segmentation networks achieved promising results in all evaluated datasets (i.e., BioSec, CasiaI3, CasiaT4, IITD-1) of NIR images and (NICE.I, CrEye-Iris and MICHE-I) of VIS images in both non-cooperative and cooperative domains, outperforming the baselines techniques which are the best ones found so far in the literature, i.e., a new state of the art for these datasets. Furthermore, we manually labeled 2,431 images from CasiaT4, CrEye-Iris and MICHE-I datasets, making the masks available for research purposes.

==> network.tex <==
\section{Network Architecture}
\label{sec:network}

\begin{figure*}[!t]
	\begin{center}
		\includegraphics[width=\linewidth]{figs/architecture.eps}
	\end{center}
	\caption{\gls*{dcnn} architecture for iris segmentation.}
	\label{fig:architecture}
\end{figure*}

In this section, we describe the \gls*{dcnn} used in our iris segmentation approach (see Figure~\ref{fig:architecture}).
An image is provided as input to the \gls*{dcnn} and a mask is generated at the output.
This mask is a binary image (of the same size) where each pixel is classified as iris or not iris.
We do not perform resize on the input image, as in~\cite{teichmann_2016_multinet}, since images of different datasets have different sizes ($W \times H \times C$) and aspect ratios, and this may impair the system performance.

Basically, we employ the MultiNet~\cite{teichmann_2016_multinet} segmentation decoder without the classification and detection decoders.
The encoder consists of the first $13$ layers of the VGG-$16$ network~\cite{Simonyan_2014_vgg16}. The features extracted from its 5th pooling~layer are then utilized by the segmentation decoder, which follows the \gls*{fcn} architecture~\cite{Shelhamer_2015_CVPR}.

The fully-connected layers of the VGG-$16$ network are transformed into $1 \times 1$ convolutional layers to produce a low-resolution segmentation.
Then, three transposed convolution layers are used to perform up-sampling.
Finally, high-resolution features are extracted through skip layers from lower layers to improve the up-sampled results.

The segmentation loss function is based on the cross-entropy.
The pre-trained VGG-$16$ weights on the ImageNet dataset~\cite{Krizhevsky_2012_ImageNet} 
are used to initialize the encoder and segmentation decoder, as well as the transposed convolutional layers.
The training is based on the Adam optimizer algorithm~\cite{kingma_adam_optimizer_2014}, with the following parameters: learning rate of $1^{-5}$, dropout probability of $0.5$, weight decay of $5^{-4}$ and standard deviation of $1^{-4}$ to initialize the skip layers.


